Balancing Efficiency and Flexibility for DNN Acceleration via Temporal GPU-Systolic Array Integration

The research interest in specialized hardware accelerators for deep neural networks (DNN) spikes recently owing to their superior performance and efficiency. However, today's DNN accelerators primarily focus on accelerating specific "kernels" such as convolution and matrix multiplication, which are vital but only part of an end-to-end DNN-enabled application. Meaningful speedups over the entire application often require supporting computations that are, while massively parallel, ill-suited to DNN accelerators. Integrating a general-purpose processor such as a CPU or a GPU incurs significant data movement overhead and leads to resource under-utilization on the DNN accelerators. We propose Simultaneous Multi-mode Architecture (SMA), a novel architecture design and execution model that offers general-purpose programmability on DNN accelerators in order to accelerate end-to-end applications. The key to SMA is the temporal integration of the systolic execution model with the GPU-like SIMD execution model. The SMA exploits the common components shared between the systolic-array accelerator and the GPU, and provides lightweight reconfiguration capability to switch between the two modes in-situ. The SMA achieves up to 63% performance improvement while consuming 23% less energy than the baseline Volta architecture with TensorCore.

==> tex/background.tex <==

    
\section{Background}
\label{sec:background}


In this section, we describe the popular hardware accelerators for accelerating regular DNN models.
We then explain the emerging hybrid models that current accelerators cannot execute efficiently.

  
\subsection{Accelerating Regular DNN Models}
\label{subsec:regular_dnn}


DNN models have recently achieved state-of-the-art results in many important domains.
Owing to their increasing popularity and high computation requirement, computer architects have started to build specialized hardware accelerators.
However, most of the existing work focused on the regular DNN models, which we refer to the most commonly used models, such as convolution neural network~\cite{krizhevsky2012imagenet} (CNN) in the computer vision domain, and multi-layer perceptron (MLP)~\cite{gardner1998artificial}, recurrent neural network (RNN)~\cite{mikolov2010recurrent}, and long short term memory (LSTM)~\cite{hochreiter1997long} in the natural language processing domain.

\begin{figure}[t]
    \includegraphics[width=\columnwidth]{figures/cnn.pdf}
    \caption{Computation of a convolutional (CONV) layer~\cite{7551407}.}
    \label{fig:cnn}
  \end{figure} 
 
 The major component of CNN models is the convolutional layer shown in \Fig{fig:cnn}, which can take up over 90\% time in the overall computations~\cite{sze2017efficient}.
CNN models use CONV layers to extract high-level features as images have information locality.
The following equation formally describes a CONV layer:
\begin{eqnarray*}
   O^{E \times F}=B^{E \times F}+\sum_{k=1}^n K^{R \times S} \circledast I_k^{H \times W} \\  
   C[e][f]=\sum_{r=1}^R \sum_{s=1}^S K[r][s]\times I[e+r][f+s]
 \end{eqnarray*}
 where $O$ is the output feature map, $B$ is the bias matrix, $K$ is the filter and $I_k$ is the $k^{th}$ input feature map. 
The CNN model has been evolving fast with deeper layers for better accuracy, e.g., LeNet~\cite{lecun1989backpropagation}, AlexNet~\cite{krizhevsky2012imagenet}, and ResNet~\cite{he2016deep}. 

Computer architects have proposed various accelerator designs with different types of dataflow for accelerating the CONV operation.
The dataflow can be categorized to four types: weight stationary, output stationary, row stationary, and no stationary. 
Weight stationary (e.g., NeuFlow~\cite{farabet2011neuflow}) holds the weight (filter) elements in processing elements (PEs), and input feature maps flow through the PE array.
In consrast, Eyeriss~\cite{7551407} with row stationary dataflow proposes to hold the entire row of the filter.
The output stationary accelerator (e.g., ShiDianNao~\cite{7284058}) accumulates output feature map elements within each PE to reduce the partial sum movement cost. 

Other models (i.e., MLP and RNN/LSTM) are heavily used in the NLP domain, which are also the dominant workloads in Google's datacenter~\cite{jouppi2017datacenter}.
We refer to the other literatures for a detailed review~\cite{mikolov2010recurrent, sak2014long}. 
The core computation of those models is the general matrix-matrix multiplication (GEMM), which the convolution operation can also be converted to through the \benchmark{img2col}~\cite{chetlur2014cudnn}.
In this sense, the GEMM accelerator has more flexibility than the direct convolution accelerator.
As such, existing commercially available GEMM accelerators such as Google's TPU~\cite{Google2018TPU,jouppi2017datacenter} and NVIDIA's Tensor Core~\cite{choquette2018volta} choose to accelerate the GEMM operation.

\begin{figure}[t]
  \hspace{0.3cm}
    \includegraphics[width=0.9\columnwidth]{figures/tpu_tc.pdf}
    \caption{TPU and TC comparison.}
    \label{fig:tpu_tc}
  \end{figure}
 
 
The TPU in \Fig{fig:tpu_tc} is based on the two-dimensional weight stationary systolic array~\cite{kung1982systolic}. Each processing element (PE) in the array performs a multiply-add (MAC) operation, where an element in the weight matrix is held stationary.
Each PE passes an element in input matrix to its bottom neighbor and the partial sum to its right neighbor.
As a result, only the PEs at the top side reads from input buffer (called activation buffer in TPU) and the ones at the right side writes to the output buffer (called accumulator).
According to Flynn's taxonomy, the systolic array is MISD (multiple instruction single data) that has a significant degree of data reuse, which translates to the reduced bandwidth requirement.
As such, the TPU-v1 can deploy a large ($256 \times 256$) systolic array.

In contrast, TensorCore (TC) is still SIMD architecture and has a limited degree of data reuse.
Each TC supports a $4 \times 4 \times 4$ GEMM operation, much smaller than the TPU architecture.
According the reverse engineered work~\cite{raihan2019modeling}, the TC executes the GEMM operation in the dot-product fashion.
Its basic building block is the 4-element dot product units (FEDP) shown in \Fig{fig:tpu_tc}, which has 4 MAC units and an adder tree.
Each TC has 16 FEDP units to support the $4 \times 4 \times 4$ GEMM operation, where each FEDP unit is assigned for the calculation of one element in the $4 \times 4$ output matrix.


    \begin{figure}
    \includegraphics[width=\columnwidth]{figures/networks.pdf}
    \caption{Mask R-CNN and DeepLab details.}
    \label{fig:maskrcnn}
   \end{figure}
   
\subsection{The Emergence of Hybrid Models}

Most of the previous work focused on designing accelerators for the regular DNN models whose core computation is the GEMM operation.
However, the algorithm field evolves so fast, which leads to the emergence of hybrid models.
Those models can have operations that cannot be executed through the GEMM, which presents significant challenges for the existing fixed-function accelerator design. 

\Fig{fig:maskrcnn} shows two such hybrid DNN models, i.e., Mask R-CNN~\cite{he2017mask} and DeepLab~\cite{chen2018deeplab}.
Both models are used for the semantic segmentation task, which aims to classify all the pixels in the input picture instead of the whole image.
Such a task is more complicated than image classification.
Thus, the state-of-the-art models rely on regular CNN models for feature extraction but also introduce additional operations beyond the scope of the regular CNN models to improve the segmentation accuracy.
As \Fig{fig:maskrcnn} shows, Mask R-CNN and Deeplab both have CNN and FC layers that are GEMM-compatible. But Mask R-CNN has \benchmark{RoIAlign}, a bi-linear interpolation that requires many reshape operations, and \benchmark{RegionProposal}, a control-flow intensive non-max suppression (NMS) algorithm.
Those operations are challenging to support with only GEMM operation.
Similarly, DeepLab has the \benchmark{ArgMax} and \benchmark{CRF} (conditional random field~\cite{lafferty2001conditional}) that are GEMM-incompatible.

==> tex/motivation.tex <==


\section{Motivation}
\label{sec:motivation}

With the development of deep learning accelerators, accelerators have gradually transitioned from specialized designs to combined generality.

%TPU shows superior performance and generality compared to other ASICs, but there are still serious performance flaws with irregular operations.
\fixme{GEMM and convolution operation experiments on TPU are demonstrated in \Tbl{tb:perf}. 
Experiment~1 executes the convolutional layer \benchmark{tf.nn.conv2d} and experiment~2 executes its corresponding GEMM operation \benchmark{tf.matmul}.
With the batch size of 1, experiment 2 runs faster than experiment 1 and TensorFlow reported automatic padding.
With the batch size of 8, experiment 1 and 2 take about the same time.
%With those two experiments, we conclude that \emph{the TPU only implements the GEMM-based convolution and it only reports the GEMM execution time without the \benchmark{img2col} overhead,} which may happen in the compiling stage. 
By the comparison, it is concluded that \emph{convolution operation is implemented as GEMM-based and the \benchmark{img2col} overhead is not included in GEMM execution time,} which may happen in the compiling stage.}

\begin{table}[t]
  %	\setlength{\abovecaptionskip}{1mm}
%    \setlength{\belowcaptionskip}{1mm}
    \centering
    \caption{Convolution layer (ResNet layer with batch $\times$ 14 $\times$ 14 $\times$ 256) execution time ($\mu s$).}
    \setlength{\tabcolsep}{1mm} 
    \renewcommand\arraystretch{1.3}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|l|c|c|c|c}
      \Xhline{1.5pt}
      \multirow{2}{*}{No.} &\multirow{2}{*}{Platforms} &\multirow{2}{*}{Kernel} & \multicolumn{2}{c|}{Batch = 1} &\multicolumn{2}{c} {Batch = 8} \\
      \cline{4-7}
      &&&Utilization&Time&Utilization&Time \\
      \hline
      1&\multirow{2}{*}{TPU} & Conv2D  & {22\%}& {89.65}&{82\%}&{89.65}\\
      
      \cline{1-1}\cline{3-7}
      2&& Matmul &  {67\%}& 14.61&{89\%}&{89.61}\\
      \Xhline{1.5pt}  

    \end{tabular}
    }
  %	\vspace{-5mm}
    \label{tb:perf}
  \end{table}

\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{figures/deep.pdf}
  \caption{Deeplab.}
  \label{fig:Deeplab} 
 \end{figure}
 
\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{figures/maskrcnn.pdf}
  \caption{Maskrcnn.}
  \label{fig:maskrcnn} 
 \end{figure}
 
\fixme{TPU run the irregular operations, such as \benchmark{argmax} and \benchmark{NMS}, on the CPU cores coming with the huge transmission overhead between host and accelerators. \Fig{fig:Deeplab} and \Fig{fig:maskrcnn} show the performance degradation of irregular operations: \benchmark{argmax} and \benchmark{NMS}. TPU also add a small SIMD lane to fit the irregular operations.}


\fixme{Nvidia choose an opposite way to increase the hardware performance with general-purpose programmability loss. They add tensor cores on the GPGPU chip independent of the SIMD lane. The tensor cores are a kind of SIMD with specific purpose and hardware layout only for GEMM.}

\fixme{\Fig{fig:tensorcore} shows the Tesla V100's tensor cores. Each SM has 8 tensor cores. Each tensor core has 64 FMA units. One warp (32 threads) is devided to 8 thread group (4 threads) and runs 2 tensor cores.  A thread group runs one Dot Product using 4 FMA units and a adder tree, which can run 4 MAC operations in one cycle. In total, one warp could run $16 \times 16 \times 16$ GEMM with 2 tensor cores, 128 FMA units. This method is specific according the hardware layout. }

\fixme{
We propose the SMA to balance efficiency with flexibility between systolic and SIMD. The SMA has more generality than TPU and three important superiority than tensor core. i) SMA is temporal integration with little extra area far less than tensor cores. SMA is more efficiency with the performance/area ratio. ii) Systolic array have advantages in data reuse and reduce the accessing to register/shared memory. SMA adopts the systolic array dataflow but the tensor core is specific SIMD. iii) The tensor core need rearrange the data in register. The SMA has little need for bandwidth, which can run SIMD and systolic array simultaneously.}
\begin{figure}[t]
\vspace*{-0.4cm}
  \includegraphics[width=\columnwidth]{figures/tensorcors.png}
  \caption{Tensor Core}
  \label{fig:tensorcore}
\vspace*{-0.5cm}
\end{figure}
